Constructing and Analyzing the LSM Compaction Design Space (Updated Version)

Log-structured merge (LSM) trees offer efficient ingestion by appending incoming data, and thus, are widely used as the storage layer of production NoSQL data stores. To enable competitive read performance, LSM-trees periodically re-organize data to form a tree with levels of exponentially increasing capacity, through iterative compactions. Compactions fundamentally influence the performance of an LSM-engine in terms of write amplification, write throughput, point and range lookup performance, space amplification, and delete performance. Hence, choosing the appropriate compaction strategy is crucial and, at the same time, hard as the LSM-compaction design space is vast, largely unexplored, and has not been formally defined in the literature. As a result, most LSM-based engines use a fixed compaction strategy, typically hand-picked by an engineer, which decides how and when to compact data. In this paper, we present the design space of LSM-compactions, and evaluate state-of-the-art compaction strategies with respect to key performance metrics. Toward this goal, our first contribution is to introduce a set of four design primitives that can formally define any compaction strategy: (i) the compaction trigger, (ii) the data layout, (iii) the compaction granularity, and (iv) the data movement policy. Together, these primitives can synthesize both existing and completely new compaction strategies. Our second contribution is to experimentally analyze 10 compaction strategies. We present 12 observations and 7 high-level takeaway messages, which show how LSM systems can navigate the compaction design space.

==> 3.5-analysis.tex <==
\Paragraph{Compaction: The Internal DB-Operation}
LSM-Trees periodically re-organize the data storage layout for the disk-resident tree component, through compactions.
Compactions sort-merge the contents of immutable files from adjacent levels and write back the updated content to disk as a new set of immutable files. 
Note that, while ingestion and queries to an LSM-based engine are driven by the \textit{external} applications connected to the database, compactions are \textit{internal} operations of an engine, the purpose of which is re-organize the data on disk to facilitate future point and range reads on the data and reduce space amplification. 





\Paragraph{Compactions Drive Performance}
Compactions affect the write amplification, write throughput, point and range lookup performance, space amplification, as well as the delete performance, and thereby, the overall performance of an LSM-based data store.
Any data movement during compaction are due to the database's internal organization, and thus, can be seen as unnecessary, contributing to write amplification. 
Also, for different compaction strategies, the cumulative bytes of data written to the disk varies widely, which causes a significant difference in the overall write throughput. 
In addition to write performance, the \blue{data layout}, compaction granularity, and especially, the data movement policy affect the locality of data in an LSM-tree, which influences both the point and range lookup performance. 
In addition, the \blue{data layout} and data movement policy heavily influences space amplification and delete performance of an LSM-based store engine. 


In this section, we discuss the implications of the different compaction strategies on the overall performance of a system, and for different key-value workloads. 

\Paragraph{Model Details}
We assume an LSM-tree with size ratio $T$, that stores $N$ entries across $L+1$ levels. 
The size of the memory buffer is $M = P \cdot B \cdot E$, where $P$ is the number of disk pages in the buffer, $B$ is the number of entries per page, and $E$ is the average size (in bytes) of a key-value entry. 
The capacity of this tree is given by $\sum_{i=0}^L M \cdot T^i$, where $M \cdot T^i$ is the capacity of Level $i$. 
Level $0$ refers to in-memory buffer, and the number of tree-levels on disk, thus, can be computed as $L = \left\lceil log_T \left( \tfrac{N}{P \cdot B} \cdot \tfrac{T-1}{T} \right) \right\rceil$.
Each sorted run in the tree is a collection of immutable sorted files. 
For simplicity, we assume each file to be of the same size as the memory buffer. 
Note that, this does not affect the scope nor the correctness of the analysis, and can be simply extended to the case where file sizes are larger than (typically a multiple of) the buffer size. 
While the capacity of a leveled or tiered level is always identical, each level has a single sorted run for leveling and may have up to $T$ sorted runs for tiering. 
To facilitate lookups, Bloom filters are maintained for each sorted file and fence pointers are retained at a granularity of disk pages. 
The amount of memory (and disk space) taken up by Bloom filters is given as $BPK \cdot N$ and that for fence pointers is $f \cdot \tfrac{N}{B}$, where $BPK$ denotes the bits-per-key allocated for the Bloom filter and $f$ is size of each pointer.


\subsection{Write Performance}
The primary objective of compactions is to re-organize the data stored on disk to create fewer longer sorted runs. 
However, as data on disk are stored in immutable files, in-place modifications are not supported in LSM-trees.
Each compaction job, thus, takes as input a number of immutable files that are read to memory from disk, and writes back a new set of immutable files to disk after the compaction job is completed. 
From the stand-point of a write-optimized data store, this data movement due to compaction is often classified as superfluous and causes high write amplification, which results in under-utilization of the device bandwidth and leads to poor write throughput~\cite{Raju2017}. 
Below, we discuss how the different dimensions of compactions affect the write performance, which is further summarized in Table \ref{tab:perf}.

\subsubsection{\textbf{Write amplification}} We define write amplification as the count for the number of times an entry is (re-)written without any modifications to disk during its lifetime (i.e., until it is physically deleted from the disk). 
While in an ideal write-optimized store, write amplification should be $1$ (i.e., entries are written in a log), periodic (re-)organization of data in LSM-trees leads to significantly high write amplification~\cite{Raju2017}. 

\textit{\blue{Data layout}.} In a leveled LSM-tree, every time a Level $i$ reaches its capacity, all (or a subset of) files from Level $i$ are compacted with all (or the overlapping) the files from Level $i+1$; thus, on average each entry is written $T$ times within a level which leads to an average-case write amplification of $\mathcal{O}(T \cdot L)$. 
For a tiered LSM, each level may have up to $T$ sorted runs with overlapping key-ranges; thus, each entry is written at least once per level resulting in an average-case write amplification of $\mathcal{O}(L)$. 
An $l$-leveled LSM-tree has its last $l$ levels implemented as leveled with the remaining shallower $L-l$ levels as tiering; and thus, the average-case write amplification in an $l$-leveled tree is given as $\mathcal{O}(L-l) + \mathcal{O}(T \cdot l)$. 
Similarly, for a hybrid LSM-tree, the average-case write amplification can be expressed as $\mathcal{O}(L-i) + \mathcal{O}(T \cdot i)$, where $L-i$ denotes the number of tiered levels in the tree. 

\textit{Compaction trigger.} Compaction triggers that relate to level capacity are the primary trigger in all LSM-trees, and thus, constitute the baseline for our write amplification analysis. 
Any additional triggers, such as staleness of a file, expired tombstone TTLs, space amplification, and read amplification manifests in more frequent compactions, which leads to higher write amplification. 
However, such secondary triggers often optimizes for a different performance metric, which may amortize the write amplification over time~\cite{Sarkar2020}. 

\textit{Compaction granularity.} Compaction granularity controls the average amount of data movement per compaction job, and is typically driven by the size of the immutable files. 
The granularity of compaction do not affect the write amplification, as the total amount of data compacted over time remains the same regardless of the granularity of data movement. 

\textit{Data movement policy.} The data movement policy in LSM-based storage engines is typically chosen as to optimize for a set of performance metrics, and thus, plays a crucial role on the overall performance of the engine, including write amplification. 
The average write amplification remains as $\mathcal{O}(T \cdot L)$ for leveling and $\mathcal{O}(T)$ for tiering as files are chosen for compaction at random or in a round-robin manner once a compaction job is triggered. 
However, choosing the file with the least overlap with its parent or grandparent levels optimizes for write amplification, and thus, have a reduced data movement due to compactions. 
For compaction strategies that optimize for other performance goals, such as read performance, space amplification, and delete performance, the write amplification is often measured to be higher than that of the average case. 

\subsubsection{\textbf{Write Throughput}} The write throughput of an LSM-tree is principally driven by the degree of utilization of the device bandwidth by writes. 
The bandwidth utilization, in turn, is affected by (i) any write stalls resulting from the compactions and (ii) the absolute bandwidth support provided by the device. 
While the time taken to complete a compaction job influences the frequency and amplitude of the write stalls, the overall data movement due to compaction determines the bandwidth of the device that can be used for writing the ingested data. 
Thus, for a given device, write throughput is affected by compactions in the same way as write amplification.  

\textit{\blue{Data layout}.} A leveled LSM-tree performs compactions eagerly whenever the memory buffer is full or a disk level reaches a nominal capacity. 
This triggers compactions frequently, which consumes the device bandwidth at a greater degree, and affects the write throughput adversely. 
In contrast, in tiering, compactions are less frequent and with the device bandwidth mostly free of compaction traffic, the write throughput is significantly improved. 

\textit{Compaction trigger.} In presence of secondary compaction triggers (alongside saturation-driven primary triggers), the data movement due to compactions may increase which leads to reduced write throughput. 
However, in most practical cases, additional compaction triggers this additional data movement due to compactions amortizes significantly over time, and thus, in the long run, the write amplification remains almost unaffected by the presence of secondary compaction triggers. 

\textit{Compaction granularity.} Larger compaction granularity results in long-living compaction jobs, which often leads to prolonged write stalls, and thereby, a steep drop in the write throughput for a significant duration, increasing the tail-latency for writes. 
Such latency spikes are generally infrequent, but highly prevalent in leveled LSM-trees that compacts whole levels at at time~\cite{ONeil1996}, leveled LSM-trees with partial compaction routines that compacts several files at a time, and in most tiered LSM-trees~\cite{ApacheCassandra,ApacheHBase}. 
A smaller compaction granularity amortized such latency spikes over time by performing smaller but more frequent compactions throughout the workload execution~\cite{FacebookRocksDB}. 
However, it is noteworthy that the overall amount of data movement due to compactions always remains the same regardless of the compaction granularity, and thus, the overall write throughput remains unaffected by the granularity of compactions. 
It is just that a smaller compaction granularity is free from any undesired latency spikes and write stalls, thereby ensuring bounded tail-latency for writes. 

\textit{Data movement policy.} Similarly to write amplification, the data movement policy also plays a critical role on the write throughput of a storage engine. 
Partial compaction routines that chooses the files with minimal overlap with the target level, saturates the device bandwidth with compaction traffic the least, and hence, has the highest write throughput. 
Optimizing for no or other performance metrics, on the other hand, increases the compaction traffic considerably, and thus, demonstrate a reduced throughput for writes. 

\subsubsection{\textbf{SSD Lifetime}}
\red{We might end up writing a small para on how compactions affect the lifetime of SSDs here.}

% \Paragraph{Workload}


\begin{table*}[ht]
    \centering
    \resizebox{\textwidth}{!}{%
        % \begin{tabular}{l|cc|cC{0mm}cC{0mm}|cC{0mm}cC{0mm}|cC{0mm}cC{0mm}}
        \begin{tabular}{ccl|ccccccc|ccccccc|ccccccc}
        \toprule % \Xhline{2\arrayrulewidth} 
        % HEADER-I
        \MCL{3}{c|}{\MRW{2.5}{\begin{tabular}[c]{@{}c@{}}\textbf{Compaction} \end{tabular}}}    
        & \MCL{7}{c|}{\textbf{\MRW{1}{\begin{tabular}[c]{@{}c@{}}\textbf{Workload} \end{tabular}}}}  
        & \MCL{7}{c|}{\textbf{\MRW{1}{\begin{tabular}[c]{@{}c@{}}\textbf{Workload} \end{tabular}}}}  
        & \MCL{7}{c}{\textbf{\MRW{1}{\begin{tabular}[c]{@{}c@{}}\textbf{Workload} \end{tabular}}}}   \\
        % HEADER-II
        \MCL{3}{c|}{\MRW{2.5}{\begin{tabular}[c]{@{}c@{}}\textbf{Knob} \end{tabular}}}  
        & \MCL{7}{c|}{\textbf{A}}  
        & \MCL{7}{c|}{\textbf{B}}  
        & \MCL{7}{c}{\textbf{C}}  \\   \cline{4-24} 
        % HEADER-III
        & & & Write    & PL    & SRQ    & LRQ    & SA    & WA    & DPL
            & Write    & PL    & SRQ    & LRQ    & SA    & WA    & DPL  
            & Write    & PL    & SRQ    & LRQ    & SA    & WA    & DPL \\\hline \bottomrule
        % 1. Compaction eagerness
        \MRW{5}{\rotatebox[origin=c]{90}{\textbf{Compaction}}} 
            & \MCL{1}{c|}{\MRW{5}{\hspace*{-12pt} \rotatebox[origin=c]{90}{\textbf{\blue{Data layout}}}}}
        & \MRW{1.5}{Leveling}        
        & \MRW{1.5}{\Up} & \MRW{1.5}{\Upp} & \MRW{1.5}{\Up} & \MRW{1.5}{\Dww} 
            & \MRW{1.5}{\Up} & \MRW{1.5}{--} & \MRW{1.5}{\Up}    
        & \MRW{1.5}{\Dwww} & \MRW{1.5}{\Dwww} & \MRW{1.5}{\Up} & \MRW{1.5}{\Up}    
            & \MRW{1.5}{\Dw} & \MRW{1.5}{\Dw} & \MRW{1.5}{\Dw} 
        & \MRW{1.5}{\Dwww} & \MRW{1.5}{\Up} & \MRW{1.5}{\Up} & \MRW{1.5}{\Upp} 
            & \MRW{1.5}{\Upp} & \MRW{1.5}{\Upp} & \MRW{1.5}{\Upp} \\ 
        
        & \MCL{1}{c|}{} 
        & \MRW{2}{Tiering}  
        & \MRW{2}{\Up} & \MRW{2}{\Upp} & \MRW{2}{\Up} & \MRW{2}{\Dww} 
            & \MRW{2}{\Up} & \MRW{2}{--} & \MRW{2}{\Up}    
        & \MRW{2}{\Dwww} & \MRW{2}{\Dwww} & \MRW{2}{\Up} & \MRW{2}{\Up}    
            & \MRW{2}{\Dw} & \MRW{2}{\Dw} & \MRW{2}{\Dw} 
        & \MRW{2}{\Dwww} & \MRW{2}{\Up} & \MRW{2}{\Up} & \MRW{2}{\Upp} 
            & \MRW{2}{\Upp} & \MRW{2}{\Upp} & \MRW{2}{\Upp} \\

        & \MCL{1}{c|}{} 
        & \MRW{2.5}{$l$-leveling} 
        & \MRW{2.5}{\Up} & \MRW{2.5}{\Upp} & \MRW{2.5}{\Up} & \MRW{2.5}{\Dww} 
            & \MRW{2.5}{\Up} & \MRW{2.5}{--} & \MRW{2.5}{\Up}    
        & \MRW{2.5}{\Dwww} & \MRW{2.5}{\Dwww} & \MRW{2.5}{\Up} & \MRW{2.5}{\Up}    
            & \MRW{2.5}{\Dw} & \MRW{2.5}{\Dw} & \MRW{2.5}{\Dw} 
        & \MRW{2.5}{\Dwww} & \MRW{2.5}{\Up} & \MRW{2.5}{\Up} & \MRW{2.5}{\Upp} 
            & \MRW{2.5}{\Upp} & \MRW{2.5}{\Upp} & \MRW{2.5}{\Upp} \\ 
            
        & \MCL{1}{c|}{} 
        & \MRW{3}{Hybrid}      
        & \MRW{3}{\Up} & \MRW{3}{\Upp} & \MRW{3}{\Up} & \MRW{3}{\Dww} 
            & \MRW{3}{\Up} & \MRW{3}{--} & \MRW{3}{\Up}    
        & \MRW{3}{\Dwww} & \MRW{3}{\Dwww} & \MRW{3}{\Up} & \MRW{3}{\Up}    
            & \MRW{3}{\Dw} & \MRW{3}{\Dw} & \MRW{3}{\Dw} 
        & \MRW{3}{\Dwww} & \MRW{3}{\Up} & \MRW{3}{\Up} & \MRW{3}{\Upp} 
            & \MRW{3}{\Upp} & \MRW{3}{\Upp} & \MRW{3}{\Upp} \\ 

        & \MCL{1}{c|}{} & & & & & & & & & & & & & & & & \\ \midrule 

        % 2. Compaction Trigger
        \MRW{6}{\rotatebox[origin=c]{90}{\textbf{Compaction}}} 
            & \MCL{1}{c|}{\MRW{6}{\hspace*{-12pt} \rotatebox[origin=c]{90}{\textbf{Trigger}}}}
        & \MRW{1.25}{\#Bytes}        
        & \MRW{1.25}{\GA} & \MRW{1.25}{\GA} & \MRW{1.25}{\GA\GA\GA} & \MRW{1.25}{\RA}   
            & \MRW{1.25}{\NA} & \MRW{1.25}{\NA} & \MRW{1.25}{\BA}    
        & \MRW{1.25}{\GA} & \MRW{1.25}{\RA} & \MRW{1.25}{\BA} & \MRW{1.25}{\BA}    
            & \MRW{1.25}{\GA} & \MRW{1.25}{\GA} & \MRW{1.25}{\GA} 
        & \MRW{1.25}{\GA} & \MRW{1.25}{\BA} & \MRW{1.25}{\BA} & 
            & \MRW{1.25}{\GA\GA} & \MRW{1.25}{\GA\GA} & \MRW{1.25}{\GA\GA} \\ 
        
        & \MCL{1}{c|}{} 
        & \MRW{1.5}{\#Files}        
        & \MRW{1.5}{\GA} & \MRW{1.5}{\GA} & \MRW{1.5}{\GA\hspace*{-1pt}\GA\hspace*{-1pt}\GA} & \MRW{1.5}{\RA}   
            & \MRW{1.5}{\NA} & \MRW{1.5}{\NA} & \MRW{1.5}{\BA}    
        & \MRW{1.5}{\GA} & \MRW{1.5}{\RA} & \MRW{1.5}{\BA} & \MRW{1.5}{\BA}    
            & \MRW{1.5}{\GA} & \MRW{1.5}{\GA} & \MRW{1.5}{\GA} 
        & \MRW{1.5}{\GA} & \MRW{1.5}{\BA} & \MRW{1.5}{\BA} & 
            & \MRW{1.5}{\GA\GA} & \MRW{1.5}{\GA\GA} & \MRW{1.5}{\GA\GA} \\
        
        & \MCL{1}{c|}{} 
        & \MRW{1.75}{\#Sorted runs}       
        & \MRW{1.75}{\GA} & \MRW{1.75}{\GA} & \MRW{1.75}{\GA\GA\GA} & \MRW{1.75}{\RA}   
            & \MRW{1.75}{\NA} & \MRW{1.75}{\NA} & \MRW{1.75}{\BA}    
        & \MRW{1.75}{\GA} & \MRW{1.75}{\RA} & \MRW{1.75}{\BA} & \MRW{1.75}{\BA}    
            & \MRW{1.75}{\GA} & \MRW{1.75}{\GA} & \MRW{1.75}{\GA} 
        & \MRW{1.75}{\GA} & \MRW{1.75}{\BA} & \MRW{1.75}{\BA} & 
            & \MRW{1.75}{\GA\GA} & \MRW{1.75}{\GA\GA} & \MRW{1.75}{\GA\GA} \\
        
        & \MCL{1}{c|}{} 
        & \MRW{2}{Staleness of file}       
        & \MRW{2}{\GA} & \MRW{2}{\GA} & \MRW{2}{\GA\GA\GA} & \MRW{2}{\RA}   
            & \MRW{2}{\NA} & \MRW{2}{\NA} & \MRW{2}{\BA}    
        & \MRW{2}{\GA} & \MRW{2}{\RA} & \MRW{2}{\BA} & \MRW{2}{\BA}    
            & \MRW{2}{\GA} & \MRW{2}{\GA} & \MRW{2}{\GA} 
        & \MRW{2}{\GA} & \MRW{2}{\BA} & \MRW{2}{\BA} & 
            & \MRW{2}{\GA\GA} & \MRW{2}{\GA\GA} & \MRW{2}{\GA\GA} \\
            
        & \MCL{1}{c|}{} 
        & \MRW{2.25}{Space amp.}         
        & \MRW{2.25}{\GA} & \MRW{2.25}{\GA} & \MRW{2.25}{\GA\GA\GA} & \MRW{2.25}{\RA}   
            & \MRW{2.25}{\NA} & \MRW{2.25}{\NA} & \MRW{2.25}{\BA}    
        & \MRW{2.25}{\GA} & \MRW{2.25}{\RA} & \MRW{2.25}{\BA} & \MRW{2.25}{\BA}    
            & \MRW{2.25}{\GA} & \MRW{2.25}{\GA} & \MRW{2.25}{\GA} 
        & \MRW{2.25}{\GA} & \MRW{2.25}{\BA} & \MRW{2.25}{\BA} & 
            & \MRW{2.25}{\GA\GA} & \MRW{2.25}{\GA\GA} & \MRW{2.25}{\GA\GA} \\ \vspace*{-2pt}
        
        & \MCL{1}{c|}{} & & & & & & & & & & & & & & & & \\ \midrule 
        % 3. Compaction Granularity
        \MRW{5}{\rotatebox[origin=c]{90}{\textbf{Compaction}}} 
        & \MCL{1}{c|}{\MRW{5}{\hspace*{-12pt} \rotatebox[origin=c]{90}{\textbf{Granularity}}}}
        & \MRW{1.5}{Level}        
        & \MRW{4}{\cmark}    & \MRW{4}{\cmark}      & {}
            & \MRW{4}{\small{\ding{109}}}   & {}    & {}  
            & {}    & \MRW{4}{\cmark}   & \MRW{4}{\small{\ding{109}}} & {}
        & {}    & \MRW{4}{\cmark} & \MRW{4}{\cmark} 
            & \MRW{4}{\cmark} & \MRW{4}{\cmark} & {} & & & & & \\ 
        
        & \MCL{1}{c|}{} 
            & \MRW{2}{File (single)}  & \Up & & & & & & & & & & & & & & \\ 

        & \MCL{1}{c|}{} 
            & \MRW{2.5}{File (multiple)} & & & & & & & & & & & & & & & \\ 
            
        & \MCL{1}{c|}{} 
            & \MRW{3}{Sorted run}      & {}
        & {} & \cmark    & \small{\ding{109}} & \cmark & {} 
        & \cmark & {} & {} & {} 
        & {} & {} & {}   & & & & & \\ 
        & \MCL{1}{c|}{}  &  & & & & & & & & & & & & & & & \\ \midrule 
        % 4. Data Movement Policy
        \MRW{6}{\rotatebox[origin=c]{90}{\textbf{Data Movement}}} 
            & \MCL{1}{c|}{\MRW{6}{\hspace*{-12pt} \rotatebox[origin=c]{90}{\textbf{Policy}}}}
        & \MRW{1}{Round-robin}        
        & \MRW{4}{\cmark}    & \MRW{4}{\cmark}      & {}
            & \MRW{4}{\small{\ding{109}}}   & {}    & {}  
            & {}    & \MRW{4}{\cmark}   & \MRW{4}{\small{\ding{109}}} & {}
        & {}    & \MRW{4}{\cmark} & \MRW{4}{\cmark} 
            & \MRW{4}{\cmark} & \MRW{4}{\cmark} & {} & & & & & \\ 
        
        & \MCL{1}{c|}{} 
            & \MRW{1}{Least overlap}  & & & & & & & & & & & & & & & \\ 
        
        & \MCL{1}{c|}{} 
            & \MRW{1}{Coldest file} & & & & & & & & & & & & & & & \\ 
        
        & \MCL{1}{c|}{} 
            & \MRW{1}{Oldest file} & & & & & & & & & & & & & & & \\ 
            
        & \MCL{1}{c|}{} 
            & \MRW{1}{File w/ most TS}      & {}
        & {} & \cmark    & \small{\ding{109}} & \cmark & {} 
        & \cmark & {} & {} & {} 
        & {} & {} & {}   & & & & & \\ 
        & \MCL{1}{c|}{}  
            & \MRW{1}{Expired TS-TTL} & & & & & & & & & & & & & & & & \\ \midrule 
        \bottomrule
        \end{tabular}
    }
%    \vspace{-0.1in}
    \caption{Implications of compaction knobs on performance in LSM-based systems. 
    \label{tab:perf}}
    \vspace{-0.25in}
\end{table*}

\subsection{Read Performance}
The fundamental purpose of re-organizing of data on disk through compactions is to facilitate efficient point lookup and range scan operations in LSM-trees. 
However, as reads and writes have to the same device bandwidth, compactions affect the read performance for mixed workloads that have ingestion and lookups interleaved. 
Even for a read-only workload, the position of the data in the tree as well as the number of levels in the tree are affected by the compaction strategy, which in turn, affect the point and range lookup performance. Below, we present how the different dimensions of compactions affect the read performance of an LSM-tree. 

\subsubsection{\textbf{Point Lookups}} The point lookup performance of an LSM-tree is enhanced at a cost of extra main memory space that is used to store auxiliary data structures, such as Bloom filters and fence pointers. 
While Bloom filters probabilistically reduces the number of runs to be probed for a point lookup, and fence pointers ensure that we perform only a single I/O per sorted run, if the Bloom filter probe returns positive. 
Compacting files often pushes the entries in the files to a deeper level, and this may asymptotically increase the cost for lookups. 

\textit{\blue{Data layout}.} 
The average cost for a point lookup operation on an non-existing key is given as $\mathcal{O}(L \cdot e^{-BPK})$ for leveling and $\mathcal{O}(T \cdot L \cdot e^{-BPK})$ in case of tiering. 
A point lookup on an existing must always perform at least one I/O to fetch the target key, and thus, the average cost for this given as $\mathcal{O}(1 + L \cdot e^{-BPK})$ for leveling and $\mathcal{O}(1 + T \cdot L \cdot e^{-BPK})$ for leveling. 
For a hybrid design, the average lookup cost for non-existing keys becomes \red{fill in}, and similarly for lookups on existing keys. 

\textit{Compaction trigger.} Compaction triggers affect the point lookup performance insignificantly. In presence of secondary triggers, compaction jobs may become more frequent, which consumes a significant proportion of the device bandwidth. 
While this affects the point lookup throughput marginally, it constitutes a serious performance bottleneck in scan-heavy workload, about which discuss in the Section \ref{sec:4.2.2}. 

\textit{Compaction granularity.} The granularity of data movement during a compaction job affects the point lookup performance on existing keys to some extent. 
For tiered LSMs and leveled LSMs with a full compaction routine, once a Level $i$ reaches a nominal capacity, all entries from that level are compacted and moved to the Level $i+1$ (rendering Level $i$ to be empty). 
Compacting all files from a level regardless of the ``hotness'' of the file causes recently and frequently accessed files to move to lower levels of the tree, which is particularly undesirable when the goal is to maximize the read throughput. 
In contrast, partial compaction allows for choosing files for compaction while optimizing for read performance.

\textit{Data movement policy.} For partial compaction strategies, the choice of files to compact influences the performance for point lookups on existing keys significantly. 
Choosing the ``coldest'' file, i.e., the least recently accessed file compaction ensures that the frequently read files are retained in the shallower level, which reduces the average cost for point lookups. 
This improvement is becomes pronounced further for lookup-intensive workloads that has a high degree of temporality~\cite{Cao2020}, reducing the cost for point lookups on existing keys to $\mathcal{O}(1)$ in leveling and $\mathcal{O}(T)$ for tiering without any assistance from caching. 
Compaction strategies that optimizes different performance metrics, such as write amplification, space amplification, or delete performance, however, may choose a ``hot'' file for compaction, which adversely affects the lookup performance. 


\subsubsection{\textbf{Range Lookups}} \label{sec:4.2.2} 
LSM-trees support range lookups by sort-merging all the qualifying runs (partly or entirely) in memory and then returning the recent-most version of the qualifying entries. 
Range lookups benefit from fence pointers in efficiently identifying the first page of qualifying entries in each level, but are not assisted by Bloom filters. 
The cost for range lookups depend on the selectivity of the range query and the number of sorted runs in a tree. 
Compactions affect the range lookup performance very differently from point lookups. 
For our analysis, we distinguish a short range lookup from long range lookup in terms of the number of disk pages per sorted run affected by the range query. 
A short range query should not have more than two qualifying pages for each sorted run present in a tree~\cite{Dayan2018}. 

\textit{\blue{Data layout}.} \blue{The data layout} controls the number of sorted runs in an LSM-tree, and therefore, influences the cost for range lookups. 
The average cost for a long range lookup is given as $\mathcal{O}(\tfrac{s \cdot N}{B})$ for leveling, and that for tiering is $\mathcal{O}(\tfrac{T \cdot s \cdot N}{B})$, where $s$ denotes the selectivity of the range query. 
For short range queries, the average cost is simply proportional to the number of sorted runs, and is given as $\mathcal{O}(L)$ for leveling and $\mathcal{O}(T \cdot L)$ for tiering. 
For hybrid designs, the cost for range lookups fall in between that for leveling and tiering, and depends on the exact design of the tree. 

\textit{Compaction trigger.} The effect of secondary compaction triggers is pronounced on the range query performance than that on point queries. 
While the amount of data movement peer operation for a point lookup and a short range lookup are comparable, long range lookups with moderate to large selectivity read a significantly larger amount of data from the disk. 
In presence of secondary compaction triggers, compactions and long range queries contend for the same device bandwidth, which causes a drop in the read throughput. 

\textit{Compaction granularity.} A larger granularity of data movement during compaction leads to large amounts of data movement periodically, and thus, causes a drop in the lookup performance as a result of bandwidth sharing. 
However, such compactions always reduce the number of non-empty levels in a tree at least by one, and by a plurality, less frequently. 
Reduction in the number of levels in a tree, improves the range lookup performance dramatically as it mitigates reading superfluous data from disk and also requires fewer CPU-cycles for the sort-merge operation. 
In the best case, the cost for long range lookups drops down to $\mathcal{O}(s)$ for leveling and $\mathcal{O}(T \cdot s)$ for tiering, and that for short range lookups becomes $\mathcal{O}(1)$ for leveling and $\mathcal{O}(T)$ in case of tiering. 
Partial compactions, in contrast, always have a logarithmically increasing number of non-empty  levels in the tree, and thus, the cost for range lookups remains unchanged. 

\textit{Data movement policy.} As range lookups require sort-merging the records spread across all sorted runs in a tree, the position of a qualifying entry in the tree do not influence the performance of range lookups. 
Also, the data movement policies only pertain to partial compactions, where the number of non-empty levels in a tree follows a strictly increasing trend, each range lookup must always take into account qualifying entries from all tree-levels. 
Thus, the range lookup performance remains agnostic of the data movement policy. 


\subsection{Space Utilization} Following prior work~\cite{Sarkar2020}, we define space amplification as the ratio between the size of superfluous entries and the size of the unique entries in the tree. 
Mathematically, space amplification ranges between $[0, \infty)$, and that if all inserted keys are unique there is no space amplification. 
However, in as fraction of updates increase in a workload, the space amplification also increases, and it is further amplified in presence of point and range deletes in a workload. 
Compactions influence the space amplification of a tree along several dimensions. 

\textit{\blue{Data layout}.} In presence of only updates, the worst-case space amplification in a leveled LSM-tree is $\mathcal{O}(1/T)$ and $\mathcal{O}(T)$ for tiering~\cite{Dayan2018}. 
However, with the addition of deletes, the space amplification increases significantly, and is given as $\mathcal{O}(\tfrac{N}{1 - \lambda})$ for leveling and $\mathcal{O}(\tfrac{(1 - \lambda) \cdot N + 1}{\lambda \cdot T})$ for tiering, where $\lambda$ denotes is ratio of the size of a tombstone and the average size of a key-value pair~\cite{Sarkar2020}. 
The space amplification for hybrid designs lay between the two extremely, and depends heavily on the exact tree design. 

\textit{Compaction trigger.} Compactions can be triggered as a function of the overall space amplification of an LSM-tree, and is particularly useful for tiered implementations which has a higher headroom for space amplification~\cite{RocksDB2020}. 
Further, triggering compactions based on number of tombstone in a file~\cite{Dong2016} or age of the oldest tombstone contained in a file~\cite{Sarkar2020} propels the tombstones eagerly to the deeper levels of the tree, which reduces the space amplification by compacting the invalidated entries early. 

\textit{Compaction granularity.} Compacting data at a large granularity often reduces the number of non-empty levels in a tree, and in the process, arranges the data across fewer but larger and more compact sorted runs. 
For example, in tiering, once a level reaches a nominal capacity all $T-1$ sorted runs are compacted together and written as a single compact and larger run in the following level, rendering the child level empty. 
Similarly, in leveling with full compaction, every time level reaches saturation, sorted runs from one or more levels are merged with the level of larger capacity, reducing the number of sorted runs. 
Any superfluous entry from the input runs is removed during this process, which leads to reduced space amplification. 
For leveling with full compactions, periodically all levels are merged together to a single long level (when the saturation trigger for all levels are triggered simultaneously), which yields a compact tree with no space amplification. 
However, for partial compaction, as the number of sorted runs always follow a increasing trend, the worst-case space amplification remains the same. 

\textit{Data movement policy.} While compacting data at the granularity of a file, choosing files for compaction based on number of tombstones in a file or tombstones with an expired time-to-live the reduces the space amplification. 
However, optimizing for performance goals, such as write amplification or read throughput, do not necessarily bring down the write amplification. 


\subsection{Delete Performance} While deletes affect the performance of an LSM-based engine across several facets, here we focus on persistently deleting entries within a time-limit in order to analyze the implications of compactions from a privacy standpoint. 
To ensure timely and persistent deletion, a tombstone must participate in a compaction involving the last tree-level within the threshold time. 

\textit{\blue{Data layout}.} The average time taken to persistently delete an entry from a tree is given by $\mathcal{O}(\tfrac{T^{L-1} \cdot P \cdot B}{I})$ for leveling and $\mathcal{O}(\tfrac{T^L \cdot P \cdot B}{I})$ for tiering~\cite{Sarkar2020}, where $I$ denotes the rate of ingestion of unique entries to the database. 
Note that, while for leveling propelling the tombstone to the last level ensures persistent deletion of the target entry, in case of tiering, the tombstone must participate in a compaction involving all the sorted runs from the last level to guarantee delete persistence. 

\textit{Compaction trigger, granularity, and data movement policy.} Saturation-based compaction triggers ensure persistence of all superfluous entries in a tree every time a new level is added to a tree, but only when the compactions are performed at a granularity of levels or sorted runs. 
For partial compaction strategies, a secondary compaction trigger, that compacts files with tombstones eagerly, must be invoked to ensure delete persistence~\cite{RocksDBTS,Sarkar2020}. 
Otherwise, in the worst-case, deletes may not be persisted at all in an LSM-tree based on partial compactions.  


\subsection{Summarizing the Implications}
\red{A super-short summary of the section.}


==> 7-related_work.tex <==

\blue{\Paragraph{LSM-trees.} 
LSM-trees exhibit excellent ingestion performance and thus have achieved tremendous success in industry~\cite{FacebookRocksDB,GoogleLevelDB,ApacheCassandra,WiredTiger,Huang2019}. As more dedicated LSM architectures \cite{Dayan2019,Raju2017} are proposed, the LSM-tree designing space becomes more complicated. 
Dayan \textit{et al.}~\cite{Dayan2018a,Dayan2018} gives an asymptotically worst-case complexity analysis for both read and write operations in LSM-trees. 
Luo and Carey~\cite{Luo2018} provides a general taxonomy to classify LSM-trees. 
Idreos \textit{et al.}~\cite{Idreos2019} proposes a design continuum to connect all existing data structures based on a fundamental set of design principles. 
However, none of them focus on the compaction strategy comparison which leaves the compaction design space largely unexplored.} 

\blue{\Paragraph{Other index structures.} 
In addition to LSM-trees, there are other backend index structures for key-value stores and they can outperform LSM-trees under some specific workloads. For instance, the big $B$-tree family, including $B^{+}$-tree, $B^{*}$-tree~\cite{Comer1979,Knuth1998}, $B^{\epsilon}$-tree~\cite{Brodal2003,Papagiannis2016}, usually provides better range lookup performance relative to traditional LSM-trees. Another type of index structure, Log-Structured Hash-table ~\cite{Sheehy2010,Chandramouli2018}, offers even faster ingestion rate than LSM-trees but they suffer from a significant performance degradation in terms of range queries. }
  

==> Makefile <==
whoami := $(shell whoami)
target := paper
latex := pdflatex
bibtex := bibtex

.PHONY: default
default: all 

.PHONY: all
all:
	$(MAKE) checkbib $(target).pdf cleanmost

checkbib: 
	sh ./get_bib.sh

%.pdf: %.tex $(wildcard *.tex) 
	$(latex) $<
	$(bibtex) $*
	$(latex) $<
	$(latex) $<

one:
	$(latex) $(target).tex

bib:
	$(bibtex) $(target)

.PHONY: clean
clean:
	make cleanmost
	rm -f $(patsubst %,%.fls,$(target)) \
	$(patsubst %,%.out,$(target)) \
	$(patsubst %,%.fdb_latexmk,$(target)) \
	$(patsubst %,%.synctex*,$(target)) \
	$(patsubst %,%.synctex.gz,$(target))

.PHONY: cleanmost
cleanmost:
	rm -f *~ *.bak \
	$(patsubst %,%.dvi,$(target)) \
	$(patsubst %,%.log,$(target)) \
	$(patsubst %,%.aux,$(target)) \
	$(patsubst %,%.bbl,$(target)) \
	$(patsubst %,%.blg,$(target)) \
	$(patsubst %,%.lox,$(target)) \
	$(patsubst %,%.upa,$(target)) \
	$(patsubst %,%.upb,$(target)) \
	$(patsubst %,%.xcp,$(target))

.PHONY: cleanall
cleanall:
	make clean
	rm -f $(patsubst %,%.pdf,$(target))

.PHONY: copy
copy:
#ifeq ($(whoami),manos)
#	rsync -a top.pdf <someshere>
#endif



